Multiple Dirichlet Series for Affine Weyl Groups

Let $W$ be the Weyl group of a simply-laced affine Kac-Moody Lie group, excepting $\tilde{A}_n$ for $n$ even. We construct a multiple Dirichlet series $Z(x_1, \ldots x_{n+1})$, meromorphic in a half-space, satisfying a group $W$ of functional equations. This series is analogous to the multiple Dirichlet series for classical Weyl groups constructed by Brubaker-Bump-Friedberg, Chinta-Gunnells, and others. It is completely characterized by four natural axioms concerning its coefficients, axioms which come from the geometry of parameter spaces of hyperelliptic curves. The series constructed this way is optimal for computing moments of character sums and L-functions, including the fourth moment of quadratic L-functions at the central point via $\tilde{D}_4$ and the second moment weighted by the number of divisors of the conductor via $\tilde{A}_3$. We also give evidence to suggest that this series appears as a first Fourier-Whittaker coefficient in an Eisenstein series on the twofold metaplectic cover of the relevant Kac-Moody group. The construction is limited to the rational function field $\mathbb{F}_q(t)$, but it also describes the $p$-part of the multiple Dirichlet series over an arbitrary global field.

==> bib.tex <==
@Article{B,
author = {B.J. Birch},
title = {How the number of points of an elliptic curve over a fixed prime field varies},
journal = {J. London Math. Soc.},
year = {1968},
OPTkey = {•},
OPTvolume = {s1-43},
OPTnumber = {1},
OPTpages = {57-60},
OPTmonth = {•},
OPTnote = {•},
OPTannote = {•}
}

@Book{Bo,
ALTauthor = {N. Bourbaki},
ALTeditor = {•},
title = {Lie Groups and Lie Algebras, Chapters 4-6},
publisher = {Springer-Verlag},
year = {2002},
OPTkey = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {Elements of Mathematics},
OPTaddress = {Berlin},
OPTedition = {•},
OPTmonth = {•},
OPTnote = {•},
OPTannote = {•}
}

@Article{BK
author = {A. Braverman and D. Kazhdan},
title = {The spherical Hecke algebra for affine Kac-Moody groups I},
journal = {Ann. of Math},
year = {2011},
OPTkey = {•},
OPTvolume = {(2) 174},
OPTnumber = {3},
OPTpages = {1603-1642},
OPTmonth = {•},
OPTnote = {•},
OPTannote = {•}
}

%\bibitem{BGKP} A. Braverman, H. Garland, D. Kazhdan, M. Patnaik, \textit{An affine Gindikin-Karpelevic formula,} preprint.

%\bibitem{BBF1} B. Brubaker, D. Bump, S. Friedberg, \textit{Weyl group multiple Dirichlet series, Eisenstein series and crystal bases,} Ann. of Math. (2) 173 2011, no. 2, 1081–1120. 

%\bibitem{BBF2} B. Brubaker, D. Bump, S. Friedberg, \textit{Weyl Group Multiple Dirichlet Series: Type A Combinatorial Theory,} Ann. of Math. Studies, 175. Princeton University Press, Princeton, NJ, 2011.

%\bibitem{BrFH} B. Brubaker, S. Friedberg, J. Hoffstein, \textit{Cubic twists of GL(2) automorphic L-functions,} Invent. Math. 160  no. 1, 2005, 31-58. 

%\bibitem{BD} A. Bucur, A. Diaconu, \textit{Moments of Quadratic Dirichlet L-functions over Rational Function Fields,} Moscow Math. J. 10, 2010, no. 3, 485-517.

%\bibitem{BFH1} D. Bump, S. Friedberg, J. Hoffstein, \textit{A nonvanishing theorem for derivatives of automorphic L-functions with applications to elliptic curves,} Bulletin of the Amer. Math. Soc. 21, no. 1, 1989, 89-95.

%\bibitem{BFH2} D. Bump, S. Friedberg, J. Hoffstein, \textit{Sums of twisted GL(3) automorphic L-functions,} Contributions to automorphic forms, geometry, and number theory, Johns Hopkins Univ. Press, Baltimore, MD, 2004, 131-162.

%\bibitem{BFH3} D. Bump, S. Friedberg, J. Hoffstein, \textit{On some applications of automorphic forms to number theory,} Bull. Amer. Math. Soc. 33, no. 2, 1996, 157-175

%\bibitem{CG1}  G. Chinta, P. E. Gunnells. \textit{Weyl group multiple Dirichlet series constructed from quadratic characters,} Invent. Math. 167, 2007, no. 2, 327–353.

%\bibitem{CG2} G. Chinta, P.E. Gunnells. \textit{Constructing Weyl group multiple Dirichlet series,} J. Amer. Math. Soc. 23, 2010, no. 1, 189–215.

%\bibitem{CFKRS} J.B. Conrey, D.W. Farmer, J.P. Keating, M. Rubinstein, N. Snaith, \textit {Integral moments of $L$-functions,} Proc. London Math. Society 91, 2005, 33-104.

%\bibitem{D1} P. Deligne \textit{La conjecture de Weil: I,}. Publications Mathématiques de l'IHÉS 43, 1974, 273–307.

%\bibitem{D2} P. Deligne \textit{La conjecture de Weil: II,} Publications Mathématiques de l'IHÉS 52, 1980, 137–252.

%\bibitem{DGH} A. Diaconu, D. Goldfeld, J. Hoffstein, \textit{Multiple Dirichlet Series and Moments of Zeta and L-functions,} Compositio Math. 139, 2003, no. 3, 297-360.

%\bibitem{DP} A. Diaconu, V. Pasol, \textit{Trace formulas, character sums, and multiple Dirichlet series,} preprint.

%\bibitem{FF1} B. Fisher, S. Friedberg, \textit{Sums of Twisted GL(2) L-functions over Function Fields}, Duke Math. J. 117, 2003, no. 3, 543-570.

%\bibitem{FF2} B. Fisher, S. Friedberg, \textit{Double Dirichlet series over Function Fields,} Compositio Math. 140, 2004, no. 3, 613-630.

%\bibitem{FZ} S. Friedberg, L. Zhang, \textit{Eisenstein series on covers of odd orthogonal groups,} preprint.

%\bibitem{G} H. Garland, \textit{Certain Eisenstein series on loop groups: convergence and the constant term,} Algebraic groups and arithmetic, Tata Inst. Fund. Res., Mumbai, 2004, 275-319.

%\bibitem{GMP} H. Garland, M. Patnaik, S. Miller \textit{Entirety of Cuspidal Eisenstein Series on Loop Groups,} preprint.

%\bibitem{GH} D. Goldfeld, J. Hoffstein, \textit{Eisenstein Series of 1/2 integral weight and the mean value of real Dirichlet L-series,} Invent. Math. 80, 1985, no. 2, 185-208.

%\bibitem{HR} J. Hoffstein, M. Rosen, \textit{Average values of L-series in function fields,} J. Reine Agnew. Math. 426, 1992, 117-150.

%\bibitem{H} J.E. Humphreys, \textit{Reflection Groups and Coxeter Groups,} Cambridge Studies in Advanced Mathematics vol. 29, Cambridge University Press, Cambridge, UK, 1990.

%\bibitem{J} M. Jutila, \textit{On the mean values of $L(\frac{1}{2}, \chi)$ for real characters,} Analysis 1, no. 2, 1981, 149-161.

%\bibitem{KS} N. Katz, P. Sarnak, \textit{Random matrices, Frobenius Eigenvalues, and Monodromy,} Amer. Math. Soc. Colloquium Publications, Providence, RI, 1999.

%\bibitem{LZ} K.H. Lee, Y. Zhang, \textit{Weyl group multiple Dirichlet series for symmetrizable Kac-Moody root systems,} preprint.

%\bibitem{M} I.G. Macdonald, \textit{Affine Root Systems and Dedekind's $\eta$-function}, Invent. Math. 15, 1972, 91-143. 

%\bibitem{R} M. Rosen, \textit{Number Theory in Function Fields,} Graduate Texts in Mathematics vol. 210, Springer-Verlag, New York, NY, 2002.

%\bibitem{S} C.L. Siegel, \textit{The average measure of quadratic forms with given determinant and signature,} Gesammelte Abhandlungen II, Springer, Berlin-Heidelburg-New York, 1966, 473-491.

%\bibitem{So} K. Soundararajan, \textit{Nonvanishing of quadratic Dirichlet L-functions at $s=\frac{1}{2}$}, Ann. of Math. 152, no.2, 2000, 447-488.
